Integrating Present and Past in Unsupervised Continual Learning

We formulate a unifying framework for unsupervised continual learning (UCL), which disentangles learning objectives that are specific to the present and the past data, encompassing stability, plasticity, and cross-task consolidation. The framework reveals that many existing UCL approaches overlook cross-task consolidation and try to balance plasticity and stability in a shared embedding space. This results in worse performance due to a lack of within-task data diversity and reduced effectiveness in learning the current task. Our method, Osiris, which explicitly optimizes all three objectives on separate embedding spaces, achieves state-of-the-art performance on all benchmarks, including two novel benchmarks proposed in this paper featuring semantically structured task sequences. Compared to standard benchmarks, these two structured benchmarks more closely resemble visual signals received by humans and animals when navigating real-world environments. Finally, we show some preliminary evidence that continual models can benefit from such realistic learning scenarios.

==> tables/_norm.tex <==
\begin{table}[t]
\caption{
KNN accuracy of methods trained on the 20-task Split-CIFAR-100 with BatchNorm (BN) or GroupNorm (GN). \texttt{1st-Only} denotes an offline model trained for the same number of steps but only on the first task. Numbers in parentheses denote improvement over \texttt{FT}. The incompatibility between BN and UCL can be mitigated by using GN instead. This allows models' ability to tackle
the core challenges of UCL
to be more clearly reflected by \texttt{FT} $\Delta$.
}
\label{tab:norm}
\begin{center}
\resizebox{0.4\linewidth}{!}{
\begin{tabular}{l|rr|rr}
\toprule
Method & \textsc{BN} & FT $\Delta$ & \textsc{GN} &  FT $\Delta$ \\
\midrule
FT & 36.7 & & 45.6 & \\
1st-Only & 39.5 & \small{\textcolor{Green}{(+2.8)}} & 40.5 & \small{\textcolor{Red}{($-$5.1)}} \\
LUMP  & 45.4 & \small{\textcolor{Green}{(+8.7)}} & 47.7 & \small{\textcolor{Green}{(+2.1)}} \\
CaSSLe & 43.1 & \small{\textcolor{Green}{(+6.4)}} & 48.0  & \small{\textcolor{Green}{(+2.4)}} \\
Offline  & 50.3 & \small{\textcolor{Green}{(+13.6)}} & 52.5 & \textcolor{Green}{\small{(+6.9)}} \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}
